A search for $\it{\Xi}^{++}_{cc} \rightarrow D^{+} p K^{-} \pi^{+}$ decays

A search for the $\it{\Xi}^{++}_{cc}$ baryon through the $\it{\Xi}^{++}_{cc} \rightarrow D^{+} p K^{-} \pi^{+}$ decay is performed with a data sample corresponding to an integrated luminosity of 1.7 $\mathrm{fb}^{-1}$ recorded by the LHCb experiment in $pp$ collisions at a centre-of-mass energy of 13 TeV. No significant signal is observed in the mass range from the kinematic threshold of the decay to 3800 $\mathrm{MeV}/c^{2}$. An upper limit is set on the ratio of branching fractions $\mathcal{R} = \frac{\mathcal{B}(\it{\Xi}^{++}_{cc} \rightarrow D^{+} p K^{-} \pi^{+})}{\mathcal{B}(\it{\Xi}^{++}_{cc} \rightarrow \Lambda^{+}_{c} K^{-} \pi^{+}\pi^{+})}$ with $\mathcal{R} < 1.7 \hspace{2pt} (2.1) \times 10^{-2}$ at the 90% (95%) confidence level at the known mass of the $\it{\Xi}^{++}_{cc}$ state.

==> LHCb_Authorship_20-Feb-2019_arXiv.tex <==
LHCb Collaboration:
R. Aaij,
C. Abell{\'a}n Beteta,
B. Adeva,
M. Adinolfi,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
F. Archilli,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
J.J. Back,
S. Baker,
V. Balagura,
W. Baldini,
A. Baranov,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
V. Batozskaya,
B. Batsukh,
A. Battig,
V. Battista,
A. Bay,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
S. Belin,
N. Beliy,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
M.S. Bieker,
S. Bifani,
P. Billoir,
A. Birnkraut,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
V. Bocci,
O. Boente Garcia,
T. Boettcher,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
M. Boubdir,
T.J.V. Bowcock,
C. Bozzi,
S. Braun,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
E. Buchanan,
A. Buonaura,
C. Burr,
A. Bursche,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
K. Carvalho Akiba,
G. Casse,
M. Cattaneo,
G. Cavallero,
R. Cenci,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
V. Chekalina,
C. Chen,
S. Chen,
S.-G. Chitic,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
F. Cindolo,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
G. Coombs,
S. Coquereau,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
J.A. de Vries,
C.T. Dean,
W. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
M. Demmer,
A. Dendek,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
S. Didenko,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A.C. dos Reis,
A. Dosil Su{\'a}rez,
L. Douglas,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
P. Durante,
J.M. Durham,
D. Dutta,
R. Dzhelyadin,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
S. Ely,
A. Ene,
S. Escher,
S. Esen,
T. Evans,
A. Falabella,
C. F{\"a}rber,
N. Farley,
S. Farry,
D. Fazzini,
M. F{\'e}o,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
W. Funk,
E. Gabriel,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
J. Garra Tico,
L. Garrido,
D. Gascon,
C. Gaspar,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
O.G. Girard,
P. Gironella Gironell,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
C. G{\"o}bel,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
C. Gu,
E. Gushchin,
A. Guth,
Yu. Guz,
T. Gys,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
B. Hamilton,
Q. Han,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heinicke,
A. Heister,
K. Hennessy,
L. Henry,
M. He{\ss},
J. Heuel,
A. Hicheur,
R. Hidalgo Charman,
D. Hill,
M. Hilton,
P.H. Hopchev,
J. Hu,
W. Hu,
W. Huang,
Z.C. Huard,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
P. Ilten,
A. Inglessi,
A. Inyakin,
K. Ivshin,
R. Jacobsson,
S. Jakobsen,
J. Jalocha,
E. Jans,
B.K. Jashal,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
C. Khurewathanakul,
K.E. Kim,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
M. Kolpin,
R. Kopecna,
P. Koppenburg,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
M. Kozeiha,
L. Kravchuk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
G.J. Kunde,
A.K. Kuonen,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
D. Lancierini,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
R. Lef{\`e}vre,
A. Leflat,
F. Lemaitre,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
P.-R. Li,
X. Li,
Y. Li,
Z. Li,
X. Liang,
T. Likhomanenko,
R. Lindner,
F. Lionetto,
V. Lisovskyi,
G. Liu,
X. Liu,
D. Loh,
A. Loi,
I. Longstaff,
J.H. Lopes,
G. Loustau,
G.H. Lovell,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Maev,
K. Maguire,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
P.J. Marshall,
G. Martellotti,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
B. Maurin,
M. McCann,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
N. Meinert,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
E. Millard,
M.-N. Minard,
O. Mineev,
L. Minzoni,
D.S. Mitzel,
A. M{\"o}dden,
A. Mogini,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mukherjee,
M. Mulder,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
C.H. Murphy,
D. Murray,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
N.S. Nolte,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
D.P. O'Hanlon,
R. Oldeman,
C.J.G. Onderwater,
J. D. Osborn,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
B. Pietrzyk,
G. Pietrzyk,
M. Pikies,
M. Pili,
D. Pinci,
J. Pinzino,
F. Pisani,
A. Piucci,
V. Placinta,
S. Playfer,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Poslavskii,
E. Price,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Ravonel Salzgeber,
M. Reboud,
F. Redi,
S. Reichert,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
S. Ricciardi,
S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
M. Roehrken,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
J.J. Saborido Silva,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Gras,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
G. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
E.S. Sepulveda,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
A. Seuthe,
P. Seyfert,
M. Shapkin,
T. Shears,
L. Shekhtman,
V. Shevchenko,
E. Shmanin,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
I. Skiba,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.G. Smeaton,
E. Smith,
I.T. Smith,
M. Smith,
M. Soares,
l. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
A. Stocchi,
S. Stone,
S. Stracka,
M.E. Stramaglia,
M. Straticiuc,
U. Straumann,
S. Strokov,
J. Sun,
L. Sun,
Y. Sun,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
Z. Tang,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
M.J. Tilley,
V. Tisserand,
S. T'Jampens,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
D.Y. Tou,
R. Tourinho Jadallah Aoude,
E. Tournefier,
M. Traill,
M.T. Tran,
A. Trisovic,
A. Tsaregorodtsev,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
M. van Beuzekom,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
J. van Tilburg,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Vernet,
M. Veronesi,
M. Vesterinen,
J.V. Viana Barbosa,
D. Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
A. Vitkovskiy,
M. Vitti,
V. Volkov,
A. Vollhardt,
D. Vom Bruch,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
R. Waldi,
J. Walsh,
J. Wang,
M. Wang,
Y. Wang,
Z. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
C. Weisser,
M. Whitehead,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
T. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wyllie,
D. Xiao,
Y. Xie,
H. Xing,
A. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
M. Zeng,
D. Zhang,
L. Zhang,
W.C. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli

==> figs/paper/title-LHCb-PAPER.tex <==
% $Id: title-LHCb-PAPER.tex 122889 2018-08-17 17:59:55Z pkoppenb $
% ===============================================================================
% Purpose: LHCb-PAPER journal paper title page template
% Author: 
% Created on: 2010-09-25
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}
\pagenumbering{roman}

% Header ---------------------------------------------------
\vspace*{-1.5cm}
\centerline{\large EUROPEAN ORGANIZATION FOR NUCLEAR RESEARCH (CERN)}
\vspace*{1.5cm}
\noindent
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r@{\extracolsep{0pt}}}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-1.5cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{figs/lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{figs/lhcb-logo.eps}} & &}%
\\
 & & CERN-EP-2019-ZZZ \\  % ID 
 & & LHCb-PAPER-2019-YYY \\  % ID 
 & & \today \\ % Date - Can also hardwire e.g.: 23 March 2010
 & & \\
% not in paper \hline
\end{tabular*}

\vspace*{4.0cm}

% Title --------------------------------------------------
{\normalfont\bfseries\boldmath\huge
\begin{center}
% DO NOT EDIT HERE. Instead edit macro in main.tex to keep metadata correct
  \papertitle 
\end{center}
}

\vspace*{2.0cm}

% Authors -------------------------------------------------
\begin{center}
%In the footnote, replace 'paper' by 'Letter' in case of submission to PRL or PLB 
% Edit macro in main.tex to keep metadata correct
\paperauthors\footnote{Authors are listed at the end of this paper.}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
  \noindent
  A search for the decay 
  \XiccppDecayDp is performed 
  with a data sample
  corresponding to an integrated luminosity of 1.7\invfb
  recorded by the LHCb experiment
  in $\proton\proton$ collisions
  at centre-of-mass energy of 13\tev.
  No significant signal is observed in the 
  mass range 3300--3800\mevcc.
  An upper limit is set on the ratio of branching fractions
  $\mathcal{R} =  \frac{\mathcal{B}(\Xiccpp \to \Dp \proton \Km \pip)}{\mathcal{B}(\Xiccpp \to \Lcp \Km \pip \pip)} $
  with 
  $\mathcal{R} < 1.5 \hspace{2pt} (1.9) \times 10^{-2}$ 
  at the 90\% (95\%) confidence level,
  including statistical and systematic uncertainties.
\end{abstract}

\vspace*{2.0cm}

\begin{center}
 To be submitted to JHEP.
\end{center}

\vspace{\fill}

{\footnotesize 
% Edit macro in main.tex to keep metadata correct
\centerline{\copyright~\papercopyright. \href{\paperlicenceurl}{\paperlicence}.}}
\vspace*{2mm}

\end{titlepage}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}
%\newpage
%
%% Author List ----------------------------
%%  You need to get a new author list!
%\input{LHCb_authorlist_2017-02-06}
%
%The author list for journal publications is provided by the Membership Committee shortly after 'approval to go to paper' has been given.
%%It will be made available on the page
%%\verb!http://www.physik.uzh.ch/~strauman/forMemCo/LHCb-PAPER-XXXX-XXX/! .
%It will be sent to you by email shortly after a paper number has beens assigned.
%The author list should be included already at first circulation, 
%to allow new members of the collaboration to verify whether they have been included correctly.
%Occasionally a misspelled name is corrected or associated institutions become full members.
%In that case, a new author list will be sent to you.
%In case line numbering doesn't work well after including the authorlist, try moving the \verb!\bigskip! after the last author to a separate line.
%
%
%The authorship for Conference Reports should be ``The LHCb
%  collaboration'', with a footnote giving the name(s) of the contact
%  author(s), but without the full list of collaboration names.


\cleardoublepage









==> fixed-symbols-def.tex <==
%%% $Id: $
%%% ======================================================================
%%% Purpose: Private fixes, alternatives, and additions to standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes.  Private modifications by P. Spradlin.
%%% Maintainer : 
%%% =======================================================================

%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
%%% BaBar macro used by BaBar.
%%%\def\babar  {\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em B\kern-0.1em{\smaller A\kern-0.2em R}}}

%% LHCb sub-detectors and sub-systems


%%% Upright (not slanted) Particles


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles


%% Leptons

%% Gauge bosons and scalars

%% Quarks

%% Light mesons

%% Heavy mesons

%% Onia

%% Baryons

%%% Missing cc versions of base macros
\def\DeltaOrDeltabar  {\kern 0.18em\optbar{\kern -0.18em \PDelta}{}\xspace}
\def\XiOrXibar        {\kern 0.18em\optbar{\kern -0.18em \PXi}{}\xspace}
\def\SigmaOrSigmabar  {\kern 0.18em\optbar{\kern -0.18em \PSigma}{}\xspace}
\def\OmegaOrOmegabar  {\kern 0.18em\optbar{\kern -0.18em \POmega}{}\xspace}


%%% Alternate and additional macros for charmed baryons
\def\Lcp          {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcm          {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Lcpm         {{\ensuremath{\LorLbar{}^{\pm}_\cquark}}\xspace}
\def\Xicp         {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicm         {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Xicpm        {{\ensuremath{\XiOrXibar{}_\cquark^{\pm}}}\xspace}
\def\Xiczbar      {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xiczorbar    {{\ensuremath{\XiOrXibar{}_\cquark^0}}\xspace}
\def\Sigmacpp     {{\ensuremath{\Sigmares^{++}_\cquark}}\xspace}
\def\Sigmacmm     {{\ensuremath{\Sigmaresbar{}^{--}_\cquark}}\xspace}
\def\Sigmacpmpm   {{\ensuremath{\SigmaOrSigmabar{}^{\pm\pm}_\cquark}}\xspace}
\def\Sigmacp      {{\ensuremath{\Sigmares^{+}_\cquark}}\xspace}
\def\Sigmacm      {{\ensuremath{\Sigmaresbar{}^{-}_\cquark}}\xspace}
\def\Sigmacpm     {{\ensuremath{\SigmaOrSigmabar{}^{\pm}_\cquark}}\xspace}
\def\Sigmacz      {{\ensuremath{\Sigmares^{0}_\cquark}}\xspace}
\def\Sigmaczbar   {{\ensuremath{\Sigmaresbar{}^{0}_\cquark}}\xspace}
\def\Sigmaczorbar {{\ensuremath{\SigmaOrSigmabar{}^{0}_\cquark}}\xspace}
\def\Xiccbare     {{\ensuremath{\Xires_{\cquark\cquark}}}\xspace}
\def\Xiccpp       {{\ensuremath{\Xires^{++}_{\cquark\cquark}}}\xspace}
\def\Xiccmm       {{\ensuremath{\Xiresbar{}^{--}_{\cquark\cquark}}}\xspace}
\def\Xiccpmpm     {{\ensuremath{\XiOrXibar{}^{\pm\pm}_{\cquark\cquark}}}\xspace}
\def\Xiccp        {{\ensuremath{\Xires^{+}_{\cquark\cquark}}}\xspace}
\def\Xiccm        {{\ensuremath{\Xiresbar{}^{-}_{\cquark\cquark}}}\xspace}
\def\Xiccpm       {{\ensuremath{\XiOrXibar{}^{\pm}_{\cquark\cquark}}}\xspace}
\def\Omegaccp     {{\ensuremath{\Omegares^{+}_{\cquark\cquark}}}\xspace}
\def\Omegaccm     {{\ensuremath{\Omegaresbar{}^{-}_{\cquark\cquark}}}\xspace}
\def\Omegaccpm    {{\ensuremath{\OmegaOrOmegabar{}^{\pm}_{\cquark\cquark}}}\xspace}


%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays

%% Lifetimes

%% Masses

%% EW theory, groups

%% QCD parameters

%% CKM, CP violation

%% Oscillations

%% Tagging

%% Key decay channels

%% Rare decays

%% Wilson coefficients and operators

%% Charm

%% QM


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Energy and momentum
%%% Aliases that are in the appropriate mixed case.
\def\TeV   {\tev}
\def\GeV   {\gev}
\def\MeV   {\mev}
\def\keV   {\kev}
\def\eV    {\ev}
\def\GeVc  {\gevc}
\def\MeVc  {\mevc}
\def\GeVcc {\gevcc}
\def\MeVcc {\mevcc}

%%% Versions that do not have the leading and trailing spaces
\newcommand{\TeVnosp}{\ifthenelse{\boolean{inbibliography}}{\ensuremath{~T\kern -0.05em eV}}{\ensuremath{\mathrm{Te\kern -0.1em V}}}}
\newcommand{\GeVnosp}{\ensuremath{\mathrm{Ge\kern -0.1em V}}}
\newcommand{\MeVnosp}{\ensuremath{\mathrm{Me\kern -0.1em V}}}
\newcommand{\keVnosp}{\ensuremath{\mathrm{ke\kern -0.1em V}}}
\newcommand{\eVnosp}{\ensuremath{\mathrm{e\kern -0.1em V}}}
\newcommand{\GeVcnosp}{\ensuremath{{\mathrm{Ge\kern -0.1em V\!/}c}}}
\newcommand{\MeVcnosp}{\ensuremath{{\mathrm{Me\kern -0.1em V\!/}c}}}
\newcommand{\GeVccnosp}{\ensuremath{{\mathrm{Ge\kern -0.1em V\!/}c^2}}}
\newcommand{\MeVccnosp}{\ensuremath{{\mathrm{Me\kern -0.1em V\!/}c^2}}}
\newcommand{\GeVGeVccccnosp}{\ensuremath{{\mathrm{Ge\kern -0.1em V^2\!/}c^4}}}

%% Distance and area
%%% Alternate versions of areas
\def\msq        {\ensuremath{{\mathrm{ \,m}}^2}\xspace}
\def\cmsq       {\ensuremath{{\mathrm{ \,cm}}^2}\xspace}
\def\mmsq       {\ensuremath{{\mathrm{ \,mm}}^2}\xspace}
\def\mumsq      {\ensuremath{{\,\upmu\mathrm{m}^2}}\xspace}

%%% Versions that do not have the leading and trailing spaces
\def\kmnosp     {\ensuremath{\mathrm{km}}}
\def\mnosp      {\ensuremath{\mathrm{m}}}
\def\msqnosp    {\ensuremath{{\mathrm{m}}^2}}
\def\cmnosp     {\ensuremath{\mathrm{cm}}}
\def\cmsqnosp   {\ensuremath{{\mathrm{cm}}^2}}
\def\mmnosp     {\ensuremath{\mathrm{mm}}}
\def\mmsqnosp   {\ensuremath{{\mathrm{mm}}^2}}
\def\mumnosp    {\ensuremath{{\upmu\mathrm{m}}}}
\def\mumsqnosp  {\ensuremath{{\upmu\mathrm{m}^2}}}
\def\nmnosp     {\ensuremath{\mathrm{nm}}}
\def\fmnosp     {\ensuremath{\mathrm{fm}}}
\def\barnnosp   {\ensuremath{\mathrm{b}}}
\def\mbarnnosp  {\ensuremath{\mathrm{mb}}}
\def\mubnosp    {\ensuremath{{\mathrm{\upmu b}}}}
\def\nbnosp     {\ensuremath{\mathrm{nb}}}
\def\invnbnosp  {\ensuremath{\mbox{nb}^{-1}}}
\def\pbnosp     {\ensuremath{\mathrm{pb}}}
\def\invpbnosp  {\ensuremath{\mbox{pb}^{-1}}}
\def\fbnosp     {\ensuremath{\mbox{fb}}}
\def\invfbnosp  {\ensuremath{\mbox{fb}^{-1}}}
\def\abnosp     {\ensuremath{\mbox{ab}}}
\def\invabnosp  {\ensuremath{\mbox{ab}^{-1}}}

%% Time 
%%% Aliases that are in the appropriate mixed case.
\def\MHz  {\ensuremath{{\mathrm{ \,MHz}}}\xspace}
\def\kHz  {\ensuremath{{\mathrm{ \,kHz}}}\xspace}
\def\Hz   {\ensuremath{{\mathrm{ \,Hz}}}\xspace}

%%% Versions that do not have the leading and trailing spaces
\def\secnosp  {\ensuremath{\mathrm{{s}}}}
\def\msnosp   {\ensuremath{{\mathrm{ms}}}}
\def\musnosp  {\ensuremath{{\upmu{\mathrm{ s}}}}}
\def\nsnosp   {\ensuremath{{\mathrm{ns}}}}
\def\psnosp   {\ensuremath{{\mathrm{ps}}}}
\def\fsnosp   {\ensuremath{\mathrm{fs}}}

\def\MHznosp  {\ensuremath{{\mathrm{MHz}}}}
\def\kHznosp  {\ensuremath{{\mathrm{kHz}}}}
\def\Hznosp   {\ensuremath{{\mathrm{Hz}}}}

\def\invpsnosp {\ensuremath{{\mathrm{ps^{-1}}}}}
\def\invnsnosp {\ensuremath{{\mathrm{ns^{-1}}}}}

\def\yrnosp   {\ensuremath{\mathrm{yr}}}
\def\hrnosp   {\ensuremath{\mathrm{hr}}}

%% Temperature

%% Material lengths, radiation

%% Uncertainties

%% Math
%%% Some macros for derivatives.  Defaults are inline macros.
\newcommand{\dxdy}[2]{\ensuremath{\mathrm{d}\hspace{-0.1em}#1/\mathrm{d}#2}\xspace}
\newcommand{\altdxdy}[2]{\ensuremath{\frac{\mathrm{d}\hspace{-0.1em}#1}{\mathrm{d}\hspace{-0.1em}#2}}\xspace}
\newcommand{\ddxdydz}[3]{\ensuremath{\mathrm{d}^{2}\hspace{-0.1em}#1/\mathrm{d}\hspace{-0.1em}#2\mathrm{d}\hspace{-0.1em}#3}\xspace}
\newcommand{\altddxdydz}[3]{\ensuremath{\frac{\mathrm{d}^{2}\hspace{-0.1em}#1}{\mathrm{d}\hspace{-0.1em}#2\mathrm{d}\hspace{-0.1em}#3}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
%%% Alternate versions of transverse symbols
\def\pT         {\mbox{$p_{\mathrm{ T}}$}\xspace}
\def\ET         {\mbox{$E_{\mathrm{ T}}$}\xspace}

%% PID
%%% Alternative versions of PID symbols typeset with a base macro.
\newcommand{\DLL}[2]{\ensuremath{\mathrm{DLL}_{#1#2}}\xspace}
\def\dllkpi     {\DLL{\kaon}{\pion}}
\def\dllppi     {\DLL{\proton}{\pion}}
\def\dllepi     {\DLL{\electron}{\pion}}
\def\dllmupi    {\DLL{\muon}{\pion}}

%%% Alternative versions of PID symbols as logs of likelihood ratios.
\newcommand{\LLR}[2]{\ensuremath{\log\left(\mathcal{L}_{#1}/\mathcal{L}_{#2}\right)}\xspace}
\def\dllaltkpi     {\LLR{\kaon}{\pion}}
\def\dllaltppi     {\LLR{\proton}{\pion}}
\def\dllaltepi     {\LLR{\electron}{\pion}}
\def\dllaltmupi    {\LLR{\muon}{\pion}}


%% Geometry

%% Accelerator

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
\def\genxicc      {\mbox{\textsc{GENXICC}}\xspace}
\def\genxiccone   {\mbox{\textsc{GENXICC1.0}}\xspace}
\def\genxicctwo   {\mbox{\textsc{GENXICC2.0}}\xspace}

%% Languages

%% Data processing

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies

%% Detector components, electronics

%% Chemical symbols

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%

